Subspace Perspective on Canonical Correlation Analysis: Dimension Reduction and Minimax Rates

Canonical correlation analysis (CCA) is a fundamental statistical tool for exploring the correlation structure between two sets of random variables. In this paper, motivated by recent success of applying CCA to learn low dimensional representations of high dimensional objects, we propose to quantify the estimation loss of CCA by the excess prediction loss defined through a prediction-after-dimension-reduction framework. Such framework suggests viewing CCA estimation as estimating the subspaces spanned by the canonical variates. Interestedly, the proposed error metrics derived from the excess prediction loss turn out to be closely related to the principal angles between the subspaces spanned by the population and sample canonical variates respectively. We characterize the non-asymptotic minimax rates under the proposed metrics, especially the dependency of the minimax rates on the key quantities including the dimensions, the condition number of the covariance matrices, the canonical correlations and the eigen-gap, with minimal assumptions on the joint covariance matrix. To the best of our knowledge, this is the first finite sample result that captures the effect of the canonical correlations on the minimax rates.

==> algorithm.tex <==
%!TEX root = SpikeCCA.tex
{\color{blue}[use simulation to show the algorithm is suboptimal?]}\\
\\
Though CCA vectors have closed form solution: $\pxhk=\sxh^{-\half}\hbU_{1:k}, \pyhk=\syh^{-\half}\hbV_{1:k}$, the computational cost can be unaffordable for large datasets when both $n$ and $p$ are large. The bottleneck lies in computing the whitening matrices, $\sxh^{-\half}, \syh^{-\half}$ which has computational complexity $O(np^2+p^3)$. In this section, we are going to demonstrate that when the covariance matrix $\sxy$ has low rank structure, the top $k$ dimensional CCA vectors can be obtained efficiently while still maintaining nearly  optimal statistical accuracy. 

Throughout the section, we assume $\mbox{rank}(\sxy)\leq r<<\min\{p_1, p_2\}$ where $r$ is known \textit{a priori} and propose the following algorithm.  The main intuition is that when the correlation structure is low rank, the CCA vectors actually lie in a low dimensional space which can be efficiently estimated and it turns out that the original large scale CCA problem can be solved very cheaply in this low dimensional space.  

The low rank structure on $\sxy$ is natural and has nice probabilistic latent variable interpretations as discussed in \cite{bach05} and \cite{foster08}, which basically assumes that there exists a $r$ dimensional hidden state $\bh$ such that condition on $\bh$, $\bx_1$ and $\bx_2$ are uncorrelated (normality is not required). 
\begin{algorithm}
   \caption{CCA with Low Rank Structure}
\begin{algorithmic}
   \STATE {\bfseries Input:} Data matrices: $\X\in\mathbb{R}^{n\times p_1}, \Y\in \mathbb{R}^{n\times p_2}$ ; Target dimension: $k$ ; Rank: $r$
   \STATE {\bfseries Output:} $(\h_x{\bf \Omega}_x, \h_y{\bf \Omega}_y)$
\begin{enumerate}
\item  Estimate the subspace  $\bH_x, \bH_y$: 
\begin{itemize}
\item Compute the partial-$r$ SVD: $\sxyh^r=(\sxyh)_r=\widetilde{\bU}_r\widetilde{\bD}_r\widetilde{\bV}_r^\top$
\item Obtain $\bH_x, \bH_y$ by solving equations: $\widetilde{\bU}_r=\sxh\bH_x, \widetilde{\bV}_r=\syh\bH_y$ 
\end{itemize}
\item  Dimension Reduction: $\widetilde{\s}_x=\bH_x^\top\sxh\bH_x,  \,\widetilde{\s}_Y=\bH_y^\top\syh\bH_y, \, \widetilde{\s}_{xy}=\bH_x^\top\sxyh^r\bH_y$
\item  Compute CCA in a low dimensional space: 
\begin{equation}
\begin{gathered}
({\bf \Omega}_x, {\bf \Omega}_y)=CCA(\widetilde{\s}_x, \widetilde{\s}_y, \widetilde{\s}_{xy}, k)\\
%\mbox{where}\quad \widetilde{\s}_x=\bH_x^\top\sxh\bH_x,  \,\widetilde{\s}_Y=\bH_y^\top\syh\bH_y, \, \widetilde{\s}_{xy}=\bH_x^\top\sxyh^r\bH_y
\end{gathered}
\nonumber
\end{equation}
\end{enumerate}
\end{algorithmic}
\label{Algo:CCA_lowrank}
\end{algorithm}

Surprisingly, the proposed algorithm is equivalent to a direct CCA with $\sxyh$ replaced by $\sxyh^r$. It is interesting in the sense that the error rate does not change while the computational cost can be significantly reduced using the proposed algorithm. 
\begin{theorem}
$(\bH_x{\bf \Omega}_x, \bH_y{\bf \Omega}_y)=CCA(\sxh, \syh, \sxyh^r, k)$.
\label{thm:computation}
\end{theorem}

Now ,we are going to analyze the computational complexity of the proposed algorithm. Let $T_{mult}$ be the computational complexity of the data matrices $\bX, \bY$ multiplying a vector. 
\begin{enumerate}
\item Paritial SVD is a well studied problem in the literature of matrix factorization and can be rapidly computed using Krylov-subspace methods or randomized algorithms with cost $O(T_{mult}r)$. See \cite{tropp11} for an overview. 
\item The least squares problem $\widetilde{\bU}_r=\sxh\bH_x, \widetilde{\bV}_r=\syh\bH_y$ can be solved using conjugate gradient type methods, e.g. LSQR proposed in \cite{paige1982}. In each iteration, the computational cost is $O(T_{mult}r)$. If assuming the number of iterations to achieve convergence is $N_{iter}$, the total cost will be $O(N_{iter}T_{mult}r)$. 
\item The dimension reduction step is simply matrix multiplication and the total cost is $O(T_{mult}r)$. The CCA in last step is performed on small matrices of dimension $r\times r$ and can be computed within $O(r^3)$. 
\end{enumerate}
\begin{remark}
The matrix $\sxh=\bX^\top\bX$ is not explicitly computed. In the proposed algorithm, it is only used to multiply a vector (e.g. $\sxh\bw$) which is achieved by first computing $\bz=\frac{1}{\sqrt{n}}\bX\bw$ and then $\frac{1}{\sqrt{n}}\bX^\top\bz$. The same argument also applies to $\sy, \sxy$. For general dense matrices, $T_{mult}=O(np)$ but In applications where $\bX, \bY$ have structures (e.g. sparsity), $T_{mult}$ can be much smaller. 
\end{remark}


==> highOrder.tex <==
%!TEX root = SpikeCCA.tex
In this section, we show how to control the higher order terms $\bdelta_6$ and $\bdelta_7$. The universal constants $C, C_1, c, \cdots$ might change from line to line. 
%\begin{lemma}
%\label{lemma-matrix-inequality}
%The following inequalities hold deterministically
%\begin{gather*}
%\|\sxh^{-1/2}-\bI_{p_1}\|_2\leq \|\sxh^{-1/2}\|_2\|\bI_{p_1}-\sxh\|_2\\
%\|\syh^{-1/2}-\bI_{p_2}\|_2\leq \|\syh^{-1/2}\|_2\|\bI_{p_2}-\syh\|_2\\
%\|\sxh^{-1/2} \sxyh\syh^{-1/2} -\sxy\|_2\leq  \|\bI_{p_1}-\sxh\|+ \|\sxh\|\|\bI_{p_2}-\syh\|+\|\sxyh-\sxy\|
%\end{gather*}
%\end{lemma}
Let $\bz=(\bx^\top, \by^\top)^\top$ be the concatenation of $\bx$ and $\by$. Then 
\[
\s_z=\begin{bmatrix}
\sx & \sxy\\
\syx&\sy
\end{bmatrix}=\begin{bmatrix}
\bI_{p_1} & \sxy\\
\syx&\bI_{p_2}
\end{bmatrix}, ~~\sh_z=\begin{bmatrix}
\sxh & \sxyh\\
\syxh&\syh
\end{bmatrix}.
\]
\begin{lemma}
There exists universal constant $C$ such that the following inequalities hold deterministically
\begin{gather*}
\|\sxh\|, \|\syh\|, \|\sxyh\|\leq \|\sh_z\|\\
\|\sx-\sxh\|, \|\sy-\syh\|, \|\sxy-\sxyh\| \leq \|\s_z-\sh_z\|\\
\|\hbLambda -\bLambda\|\leq \|\sxh^{-1/2} \sxyh\syh^{-1/2} -\sxy\|\leq \|\s_z-\sh_z\|\left(2+\|\sh_z\|\right)\\
\begin{aligned}
\|\pxhk^l\|, \|\pyhk^l\|
%&\leq C\|\s_z-\sh_z\|\left(2+\|\sh_z\|\right)/\Delta+\|\s_z-\sh_z\|\left(\|\pxhk\|+ \|\pyhk\|\right)\\
&\leq  C\|\s_z-\sh_z\|\left( \frac{2+\|\sh_z\|}{\Delta}+\|\pxhk\|+ \|\pyhk\|\right)
\end{aligned}
\end{gather*}
where $\Delta=\lambda_k-\lambda_{k+1}$ is the eigen-gap. 
\label{lemma-matrix-inequality}
\end{lemma}
%\begin{lemma}
%There exists universal constant $C$ such that the following inequalities hold deterministically
%\begin{gather*}
% \|\pxhk\|,  \|\pyhk\|\leq \|\sh_z\|\\
%%\|\pyhk^u\|\leq \|\pyhk\|\leq \|\syh^{\half}\|\\
%\|\pxhk^l\|, \|\pyhk^l\|\leq C\|\s_z-\sh_z\|(1+\|\sh_z\|+\|\sh_z^{-1}\|)/|\hlambda_k-\lambda_{k+1}|
%\end{gather*}
%\label{lemma-matrix-inequality2}
%\end{lemma}





==> oversampling.tex <==
%!TEX root = SpikeCCA.tex
\section{Estimation with larger sample canonical subspaces}
In the previous section, to estimate the $k$-dimensional population canonical subspaces $\text{span}(\vct{x}^\top \mtx{\Phi}_k)$ and $\text{span}(\vct{y}^\top \mtx{\Psi}_k)$, we ambitiously use the $k$-dimensional sample canonical subspaces $\text{span}(\vct{x}^\top \widehat{\mtx{\Phi}}_k)$ and $\text{span}(\vct{y}^\top \widehat{\mtx{\Psi}}_k)$. However, as we have proven in the previous section, the accuracy of the estimation depends inversely on $\Delta = \lambda_k - \lambda_{k+1}$, which in practice could be very small. In this section, we propose to estimate these population canonical subspaces with larger sample canonical subspaces, and as we will explain later, these estimations could be much more accurate and stable then using exactly $k$-dimensional subspaces.

Consider the $m$-partial SVD is defined as 
\[
\widehat{\mtx{\Sigma}}_x^{-\frac{1}{2}} \widehat{\mtx{\Sigma}}_{xy}\widehat{\mtx{\Sigma}}_y^{-\frac{1}{2}} \approx \widehat{\mtx{U}}_m \widehat{\mtx{D}}_m \widehat{\mtx{V}}_m^\top,
\]
where $m \ll \min(p_1, p_2)$ and $m > k$. Then define $\widehat{\mtx{\Phi}}_m = \widehat{\mtx{\Sigma}}_x^{-\frac{1}{2}}\widehat{\mtx{U}}_m$, and $\widehat{\mtx{\Psi}}_m = \widehat{\mtx{\Sigma}}_y^{-\frac{1}{2}}\widehat{\mtx{V}}_m$. Then the two sample canonical subspaces become $\lspan(\vct{x}^\top\widehat{\mtx{\Phi}}_m)$ and $\lspan(\vct{y}^\top\widehat{\mtx{\Psi}}_m)$. In order to measure the distance between $\text{span}(\vct{x}^\top \mtx{\Phi}_k)$ and $\lspan(\vct{x}^\top\widehat{\mtx{\Phi}}_m)$. Recall that for any subspaces $\mathcal{M}$ and $\mathcal{L}$ in a finite-dimensional Hilbert spaces, if the dimension of $\mathcal{M}$ is less than or equal to that of $\mathcal{L}$, we can define
\[
\vvvert\sin \theta(\mathcal{M}, \mathcal{L})\vvvert = \vvvert (\mtx{I} - \mtx{P}_{\mathcal{L}})\mtx{P}_{\mathcal{M}} \vvvert
\]
for any unitary invariant norm $\vvvert \cdot \vvvert$. Therefore, we can define
\[
L(\text{span}(\vct{x}^\top \mtx{\Phi}_k), \lspan(\vct{x}^\top\widehat{\mtx{\Phi}}_m)):= \| \sin \theta(\text{span}(\vct{x}^\top \mtx{\Phi}_k), \lspan(\vct{x}^\top\widehat{\mtx{\Phi}}_m)) \|_F^2.
\]
By simple calculation, we have
\begin{align*}
L(\text{span}(\vct{x}^\top \mtx{\Phi}_k), \lspan(\vct{x}^\top\widehat{\mtx{\Phi}}_m)) & = \| \sin \theta(R(\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\mtx{\Phi}_k), R(\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m)) \|_F^2
\\
& = \left\| \left(\mtx{I} - \mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} \right)\mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\mtx{\Phi}_k}\right\|_F^2
\end{align*}
We have the following theorem
\begin{theorem}
\label{thm:upper2}
Define $\Delta_{(k, m+1)}:=\lambda_k - \lambda_{m+1}$. There exists universal positive constants $c_1, c_2$ and $C$, such that if 
\[
n\geq c_1(p_1+p_2)\left(\kappa^2+ \frac{1}{\Delta_{(k, m+1)}^2}\right),
\] 
then with probability at least $1-e^{-c_2p_1} - e^{-c_2p_2}$,
\begin{equation}
\label{eq:bound2}
L\left(\lspan{\left(\vct{x}^\top\mtx{\Phi}_k\right)}, \lspan{\left(\vct{x}^\top\widehat{\mtx{\Phi}}_m\right)}\right)\leq C\frac{k}{\Delta_{(k, m+1)}^2}\frac{p_1+p_2}{n}
\end{equation}
\end{theorem}

\subsection{Proof of \prettyref{thm:upper2}}
\begin{proof}
Notice that 
\begin{align*}
\left\| \left(\mtx{I} - \mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} \right)\mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\mtx{\Phi}_k}\right\|_F 
&\leq \left\| \left(\mtx{I} - \mtx{P}_{\widehat{\mtx{\Sigma}}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} \right)\mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\mtx{\Phi}_k}\right\|_F + \left\| \left(\mtx{P}_{\widehat{\mtx{\Sigma}}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} - \mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} \right)\mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\mtx{\Phi}_k}\right\|_F
\\
&:=I_1 + I_2.
\end{align*}
Let's first bound $I_1$. Notice that
\begin{align*}
\left\| \left(\mtx{I} - \mtx{P}_{\widehat{\mtx{\Sigma}}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} \right)\mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\mtx{\Phi}_k}\right\|_F & \leq \sqrt{k}\left\| \left(\mtx{I} - \mtx{P}_{\widehat{\mtx{\Sigma}}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} \right)\mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\mtx{\Phi}_k}\right\|
\\
& = \sqrt{k} \left\|\sin \theta(R(\mtx{U}_k), R(\widehat{\mtx{U}}_m))\right\|.
\end{align*}
Notice that $\widehat{\mtx{U}}_m=\sxh^{\frac{1}{2}}\pxh_m$ and $\mtx{U}_k=\sx^{\frac{1}{2}}\px_k$ are leading left  singular vectors of $\sxh^{-\frac{1}{2}}\sxyh\syh^{-\frac{1}{2}}$ and $\sx^{-\frac{1}{2}}\sxy\sy^{-\frac{1}{2}}$ respectively. Let 
\[
\mtx{J}:= \sxh^{-\frac{1}{2}}\sxyh\syh^{-\frac{1}{2}}-\sx^{-\frac{1}{2}}\sxy\sy^{-\frac{1}{2}}
\]
By Wedin's singular vectors sin-theta theorem,
\begin{align*}
\label{proof-wedin2}
\left\|\sin \theta(R(\mtx{U}_k), R(\widehat{\mtx{U}}_m))\right\| \leq \frac{\|\mtx{J}\|}{\lambda_k-\hat{\lambda}_{m+1}}, 
\end{align*}
where $\hat{\lambda}_{m+1}$ is the $(m+1)_{th}$ largest singular value of $\sxh^{-\frac{1}{2}}\sxyh\syh^{-\frac{1}{2}}$ and $\lambda_k$ is the $k_{th}$ largest singular value of $\sx^{-\frac{1}{2}}\sxy\sy^{-\frac{1}{2}}$ (also the $k_{th}$ canonical correlation). \\
On the one hand, by Lemma \ref{lmm:perturbation}, we have
\[
\|\mtx{J}\| \leq C\sqrt{\frac{p_1 + p_2}{n}}
\]
On the other hand, by Weyl's inequality, $|\hat{\lambda}_{m+1}-\lambda_{m+1}|\leq \|\mtx{J}\|$ and when $\sqrt{\frac{p_1+p_2}{n}}\leq \frac{\Delta_{(k, m+1)}}{2C}$ 
\begin{equation}
\lambda_k-\hat{\lambda}_{m+1}\geq \Delta_{(k, m+1)} - C\sqrt{\frac{p_1+p_2}{n}}\geq \frac{\Delta_{(k, m+1)}}{2}
\nonumber
\end{equation}
Therefore, we have
\[
\left\| \left(\mtx{I} - \mtx{P}_{\widehat{\mtx{\Sigma}}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} \right)\mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\mtx{\Phi}_k}\right\|_F \leq C\frac{\sqrt{k}}{\Delta_{(k, m+1)}}\sqrt{\frac{p_1 + p_2}{n}}
\]
~\\

Now, let's bound $I_2$. Notice that
\[
\left\| \left(\mtx{P}_{\widehat{\mtx{\Sigma}}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} - \mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} \right)\mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\mtx{\Phi}_k}\right\|_F \leq \sqrt{k}\left\| \mtx{P}_{\widehat{\mtx{\Sigma}}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} - \mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} \right\|,
\]
while 
\begin{align*}
\left\| \mtx{P}_{\widehat{\mtx{\Sigma}}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} - \mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} \right\| &\leq \left\| \left(\mtx{I} - \mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} \right)\mtx{P}_{\widehat{\mtx{\Sigma}}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m}\right\| +\left\| \mtx{P}_{\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m}\left(\mtx{I} - \mtx{P}_{\widehat{\mtx{\Sigma}}_{\vct{x}}^{\frac{1}{2}}\widehat{\mtx{\Phi}}_m} \right)\right\|
\\
& = 2\left\|\sin \theta \left( R(\widehat{\mtx{U}}_m), R(\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}} \widehat{\mtx{\Phi}}_m)\right)\right\|.
\end{align*}
Notice that $\sigma_m(\widehat{\mtx{U}}_m)=1$ while $\sigma_{m+1}(\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}} \widehat{\mtx{\Phi}}_m)=0$. By Wedin's sin-theta theorem, we have
\begin{align*}
\left\|\sin \theta \left( R(\widehat{\mtx{U}}_m), R(\mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}} \widehat{\mtx{\Phi}}_m)\right)\right\| &\leq \|\widehat{\mtx{U}}_m - \mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}} \widehat{\mtx{\Phi}}_m\|
\\
& = \|\widehat{\mtx{\Sigma}}_{\vct{x}}^{\frac{1}{2}} \widehat{\mtx{\Phi}}_m - \mtx{\Sigma}_{\vct{x}}^{\frac{1}{2}} \widehat{\mtx{\Phi}}_m\|
\\
&\leq \left\|\mtx{\Sigma}_x^{\frac{1}{2}}\widehat{\mtx{\Sigma}}_x^{-\frac{1}{2}} - \mtx{I}\right\| \left\|\widehat{\mtx{U}}_m\right\|
\\
&\leq C\sqrt{\frac{p_1}{n}}
\end{align*}
In summary, \prettyref{eq:bound2} is obtained.
\end{proof}



==> proof.tex <==
%!TEX root = main.tex




\strangesection{C}{Lower Bound: Proof of Theorem~\ref{thm:lower}}
\input{lower}

\strangesection{D}{Technical Lemmas}
%\section*{Supporting Lemmas}
%\begin{lemma}(Wedin's $sin\theta$ Theorem,  \cite{wedin1972perturbation})
%Let $\bA, \bE\in \mathbb{R}^{n\times m}$ and $\bB=\bA+\bE$. Suppose
%$$\bA=\bA_1+\bA_2,\, \bB=\bB_1+\bB_2$$ 
%where $\bA_1^\top\bA_2=\bA_2^\top\bA_1=\bB_1^\top\bB_2=\bB_2^\top\bB_1=\mtx{0}$ and $\sigma_{\min}(\bA_1)\geq \alpha+\delta, \sigma_{\min}(\bB_2)\leq \alpha$. Then for every unitary invariant norm,
%\begin{equation}
%\|\sin \theta (R(\bA_1), R(\bB_1))\|\,,\,\| \sin \theta (R(\bA_1^\top), R(\bB_1^\top))\|\leq \frac{\max\big\{\| \bP_{R(\bA_1)}\bE \|, \| \bE \bP_{R(\bA_1^\top)}\|\big \}}{\delta}
%\nonumber
%\end{equation}
%\label{wedin}
%where $\|\sin\theta (R(\bA_1), R(\bB_1))\|\doteq\|(\bI-\bP_{R(\B_1)})\bP_{R(\bA_1)}\|$
%\end{lemma}
\
%\strangesection{E}{Connection with the Loss Function in \cite{gao2015minimax}}
%\label{sec::loss-gao}
%The proposed Frobenius norm loss function is upper bounded by the loss function of \cite{gao2015minimax}. Specifically, we are going to show 
%\begin{gather}
%\mc{L}_2(\lspan(\vct{x}^\top\pxk), \lspan(\vct{x}^\top\pxhk))=2\inf\limits_{\mtx{Q} \in \mathbb{R}^{k \times k}} \E\left\|\vct{x}^\top\pxk - \vct{x}^\top\pxhk\mtx{Q}\right\|^2, 
%\label{eq:fnorm-loss}
%\end{gather}
%and therefore, 
%\begin{align*}
%\inf\limits_{\mtx{Q} \in \mc{O}(k, k)}\E\left\|\vct{x}^\top\pxk - \vct{x}^\top\pxhk\mtx{Q}\right\|^2&\geq \inf\limits_{\mtx{Q} \in \mathbb{R}^{k \times k}}\E\left\|\vct{x}^\top\pxk - \vct{x}^\top\pxhk\mtx{Q}\right\|^2\\
%&\geq \frac{1}{2}\mc{L}_2(\lspan(\vct{x}^\top\pxk), \lspan(\vct{x}^\top\pxhk)).
%\end{align*}
%To prove \eqref{eq:fnorm-loss}, simple algebra yields
%\begin{align*}
% \E\left\|{\bx}^\top \pxk-{\bx}^\top\pxhk\mtx{Q}\right\|_2^2&=\trace \left((\pxk-\pxhk\mtx{Q})^\top\mtx{\Sigma}_x(\pxk- \pxhk\mtx{Q})\right)\\
% &=\left\|{\sx}^{\half}\pxk- {\sx}^{\half}\pxhk\mtx{Q}\right\|_F^2.
%\end{align*}
%Then the least squares solution $\bQ^*=(\pxhk^\top\sx\pxhk)^{-1}\pxhk^\top\sx\pxk$ achieves the minimum. Substitute $\bQ^*$ into the objective will show that
%\begin{equation*}
%\begin{aligned}
%\inf\limits_{\mtx{Q} \in \mathbb{R}^{k \times k}} \left\|\sx^{\half}\pxk-\sx^{\half}\pxhk\bQ \right\|_F^2& =\left\|\left(\bI_{p_1}-\bP_{\sx^{\half}\pxhk}\right)\sx^{\half}\pxk\right\|_F^2
%\end{aligned}
%\end{equation*} 
%Notice that $\sx^{\half}\pxk\in\mc{O}(p_1, k)$, then 
%\begin{equation*}
%\begin{aligned}
%\inf\limits_{\mtx{Q} \in \mathbb{R}^{k \times k}} \left\|\sx^{\half}\pxk-\sx^{\half}\pxhk\bQ \right\|_F^2& =\left\|\left(\bI_{p_1}-\bP_{\sx^{\half}\pxhk}\right)\sx^{\half}\pxk\left(\sx^{\half}\pxk\right)^\top\right\|_F^2\\
%&=\left\|\left(\bI_{p_1}-\bP_{\sx^{\half}\pxhk}\right)\bP_{\sx^{\half}\pxk}\right\|_F^2\\
%&= \frac{1}{2} \left\|\mtx{P}_{\sx^{\half}\pxk} - \mtx{P}_{\sx^{\half}\pxhk} \right\|_F^2.
%\end{aligned}
%\end{equation*} 
%where the last equality is due to Lemma~\ref{lemma-projection}. 

%\subsubsection{Novel hypothesis class in lower bound proof}
%\label{sec:lower_proof}
%The first reviewer raised the concern that we used the same packing lemma and Fano's inequality to establish the lower bound. Fano's lemma is very standard in lower-bound proofs and the packing lemma and its variants are developed in the PCA literature (e.g. \cite{vu2013minimax}, \cite{cai2013sparse}). We directly use the version adapted by \cite{gao2014sparse} and we have no intention to claim any credits from these tools. However, the lower bound proof is not routine calculations based on the set-up of \cite{gao2014sparse} as commented by the first reviewer. Both the parameter space and final results of our lower-bound are very different from those of \cite{gao2014sparse} in the first place. 
%
%The novelty of our lies in the construction of the hypothesis class to which the packing lemma and Fano's inequality are applied. Technically, in the set-up of \cite{gao2014sparse}, to establish the lower bound for estimating $\pxk$, it suffices to fix $\pyk$ and only consider the perturbation of $\pxk$ when constructing the hypothesis class. Such type of construction follows the same logic as what appears in the PCA literature (e.g. \cite{vu2013minimax}, \cite{cai2013sparse}). 
%
%In contrast, we establish lower bounds for a family of parameter spaces, each with fixed $\lambda_k$ and $\lambda_{k+1}$, in which case similar construction in  \cite{vu2013minimax}, \cite{cai2013sparse} or \cite{gao2014sparse} no longer suffices to obtain the eigen-gap effect $1/(\lambda_k - \lambda_{k+1})^2$ in the lower bound. We have to consider the perturbation of both $\pxk$ and $\pyk$ in the construction of the hypothesis class (see Section C.3 in the appendix for details). This is nontrivial and to the best of our knowledge, new in the literature. 
%
%
%\strangesection{A}{Proof of Theorem~\ref{thm-metric}}
%\label{section-proof-loss}
%For any $\bU_1, \bU_2\in\mathbb{R}^{p\times k}$, from classical linear model theory, 
%\[
%\bbeta_i :=\arg\min_{\bbeta}\E\left[\left|z-\bbeta^{\top} (\bU_i^\top\bx_i)\right|^2\right]=(\bU_i^\top\sx\bU_i)^{-1}\bU_i^\top\vct{\sigma}_{xz}, ~~i=1, 2, 
%\]
%and 
%\begin{align*}
%loss(z|\lspan(\bx^\top\bU_i))&=\E[z^2]-\E[(\bbeta_i^{\top} (\bU_i^\top\bx_i))^2]\\
%&=\sigma_z^2-\vct{\sigma}_{xz}^\top\bU_i(\bU_i^\top\sx\bU_i)^{-1}\bU_i^\top\sx\bU_i(\bU_i^\top\sx\bU_i)^{-1}\bU_i^\top\vct{\sigma}_{xz}\\
%&=\sigma_z^2\left(1-\br_{xz}^\top(\sx^{\half}\bU_i)(\bU_i^\top\sx\bU_i)^{-1}(\sx^{\half}\bU_i)^\top\br_{xz}\right). 
%\end{align*}
%Notice that $(\sx^{\half}\bU_i)(\bU_i^\top\sx\bU_i)^{-\half}$ has orthonormal columns with column space $\lspan(\sx^{\half}\bU_i)$, then
%\begin{align*}
%loss(z|\lspan(\bx^\top\bU_i))=\sigma_z^2\left(1-\br_{xz}^\top\bP_{\sx^{\half}\bU_i}\br_{xz}\right). 
%\end{align*}
%Therefore, 
%\begin{align*}
%loss(z|\lspan(\bx^\top\bU_1))-loss(z|\lspan(\bx^\top\bU_2))=\sigma_z^2\br_{xz}^\top\left(\bP_{\sx^{\half}\bU_2}-\bP_{\sx^{\half}\bU_1}\right)\br_{xz}. 
%\end{align*}
%By the variational definition of the leading eigenvalue, 
%\begin{align*}
%\sup\limits_{\br_{xz}: ~\|\br_{xz}\|^2=R^2} loss(z|\lspan(\bx^\top\bU_1))-loss(z|\lspan(\bx^\top\bU_2))&=\sigma_z^2R^2 \lambda_{\max} \left(\bP_{\sx^{\half}\bU_2}-\bP_{\sx^{\half}\bU_1}\right)\\
%&=\sigma_z^2R^2 \left\| \bP_{\sx^{\half}\bU_2}-\bP_{\sx^{\half}\bU_1}\right\|, 
%\end{align*}
%where the second equality is by the characterization of the difference between two projection matrices due to  \cite{wedin1983angles}.  This proves the first claim of the theorem. For the second part, since $\br_{xz}\in\mc{A}$, 
%\begin{align*}
%&loss(z|\lspan(\bx^\top\mtx{U})) - loss(z|\lspan(\bx^\top\os))\\
%&=\sigma_z^2 \br_{xz}^\top \left(\bP_{\sx^{\half}\os}-\bP_{\sx^{\half}\bU}\right)\br_{xz}\\
% &=\sigma_z^2 \br_{xz}^\top\bP_{\sx^{\half}\os} \left(\bP_{\sx^{\half}\os}-\bP_{\sx^{\half}\bU}\right)\bP_{\sx^{\half}\bU_2}\br_{xz}\\
%&= \sigma_z^2 \br_{xz}^\top\bP_{\sx^{\half}\os} \left(\bI_{p}-\bP_{\sx^{\half}\bU}\right)\bP_{\sx^{\half}\os}\br_{xz}\\
%&\leq \sigma_z^2 R^2\left\|\bP_{\sx^{\half}\os} \left(\bI_{p}-\bP_{\sx^{\half}\bU}\right)\bP_{\sx^{\half}\os}\right\|\\
%&=\sigma_z^2R^2 \left\|\bP_{\sx^{\half}\os} \left(\bI_{p}-\bP_{\sx^{\half}\bU}\right)\right\|^2\\
%&=\sigma_z^2R^2 \left\| \bP_{\sx^{\half}\os}-\bP_{\sx^{\half}\bU}\right\|^2. 
%\end{align*}
%Notice that $\bP_{\sx^{\half}\os} \left(\bI_p-\bP_{\sx^{\half}\bU}\right)\bP_{\sx^{\half}\os}$ is positive definite. Let $\bu_1$ be the leading singular vector of this matrix and define $\br_{xz}^*=R\bu_1$. Then $\br_{xz}^*\in\mc{A}$ and with such choice of $\br_{xz}^*$, the inequality above will become equality and this implies that 
%\begin{align*}
%\sup \limits_{\br_{xz}^*\in\mc{A}} \left\{ loss(z|\lspan(\bx^\top\mtx{U})) - loss(z|\lspan(\bx^\top\os))\right\} = \sigma_z^2 R^2 \left\|\bP_{\sx^{\half}\bU}-\bP_{\sx^{\half}\os}\right\|^2. 
%\end{align*}
%For the last part of the theorem, let $\bP_{\sx^{\half}\os}=\bQ\bQ^\top$. Then the set $\mc{A}$ can be rewritten as 
%\[
%\mc{A}=\{\br: \br=R\bQ\wt{\br}, ~\wt{\br}\in\mathbb{S}^{k-1}\}. 
%\]
%The uniform measure (Haar measure) $\pi$ on $\mc{A}$ can be defined through the uniform measure (Haar measure) $\wt{\pi}$ on the sphere $\mathbb{S}^{k-1}$. Because $\wt{\pi}$ is uniform on the sphere $\mathbb{S}^{k-1}$, then $\text{Var}(\wt{\pi})=\bI_{k}/k$ (by symmetry) and 
%\begin{align*}
%&\underset{ \br_{xz}\sim \pi}{\E}\left[ loss(z|\lspan(\bx^\top\mtx{U})) - loss(z|\lspan(\bx^\top\os))\right ]\\
%=&\sigma_z^2R^2~ \E_{\wt{r}\sim\wt{\pi}}\left[\wt{\br}^\top\bQ^\top \left(\bP_{\sx^{\half}\os}-\bP_{\sx^{\half}\bU}\right)\bQ\wt{\br} \right]\\
%=& \sigma_z^2R^2\tr\left(\bQ^\top\left( \bP_{\sx^{\half}\os}-\bP_{\sx^{\half}\bU}\right)\bQ \right)/k\\
%=&\sigma_z^2R^2\tr\left(\left( \bP_{\sx^{\half}\os}-\bP_{\sx^{\half}\bU}\right)\bQ \bQ^\top\right)/k\\
%=&\sigma_z^2R^2\tr\left(\left( \bI_{p}-\bP_{\sx^{\half}\bU}\right)\bP_{\sx^{\half}\os}\right)/k
%\end{align*}
%Notice that $\bP_{\sx^{\half}\os}=\bP_{\sx^{\half}\os}^2$, 
%\begin{align*}
%&\underset{ \br_{xz}\sim \pi}{\E}\left[ loss(z|\lspan(\bx^\top\mtx{U})) - loss(z|\lspan(\bx^\top\os))\right ]\\
%=&\sigma_z^2R^2 \tr\left(\bP_{\sx^{\half}\os} \left(\bI_p-\bP_{\sx^{\half}\bU}\right)\bP_{\sx^{\half}\os} \right)/k\\
%=& \sigma_z^2R^2\left\|\bP_{\sx^{\half}\os} \left(\bI_p-\bP_{\sx^{\half}\bU}\right)\right\|_F^2/k\\
%=&\sigma_z^2R^2\left\|\bP_{\sx^{\half}\bU}-\bP_{\sx^{\half}\os}\right\|_F^2/2k, 
%\end{align*}
%where the last equality is due to Lemma~\ref{lemma-projection}.

